Optimal Software Architecture From Initial Requirements: An End-to-End Approach

A software architect turns system requirements into a suitable software architecture through an architecture optimization process. However, how should the architect decide which quality improvement to prioritize, e.g., security or reliability? In software product line, should a small improvement in multiple products be preferred over a large improvement in a single product? Existing architecture optimization methods handle various steps in the process, but none of them systematically guides the architect in generating an optimal architecture from the initial requirements. In this work we present an end-to-end approach for generating an optimal software architecture for a single software product and an optimal family of architectures for a family of products. We report on a case-study of applying our approach to optimize five industry-grade products in a real-life product line architecture, where 359 possible combinations of ten different quality efforts were prioritized.

==> sty/gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> tex/AResults.tex <==
\pgfplotsset{width=18cm,compat=1.14}
%\resizebox{.75\textwidth}{!}{
\begin{tikzpicture}[rotate=90]
%\begin{tikzpicture}[thick, scale = 1.5]
\begin{axis}[
    ybar,
    enlargelimits=0.10,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={Weighted Score},
    symbolic x coords={Reliability,Performance efficiency, Maintainability, Portability, Security},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates{
%\addplot coordinates {
(Reliability,15.472)
(Performance efficiency,13)
(Maintainability,6.854)
(Portability,5.6)
(Security,9.75)
};
\addplot coordinates{
%\addplot coordinates {
(Reliability,12.304)
(Performance efficiency,9.25)
(Maintainability,3.946)
(Portability,16.8)
(Security,11.5)
};
\addplot coordinates{
%\addplot coordinates {
(Reliability,8.5)
(Performance efficiency,8.25)
(Maintainability,5.6)
(Portability,6.552)
(Security,4)
};
\addplot coordinates{
%\addplot coordinates {
(Reliability,16.496)
(Performance efficiency,12.5)
(Maintainability,20)
(Portability,18.6)
(Security,3.75)
};
%\addplot coordinates{
\addplot coordinates {
(Reliability,15.304)
(Performance efficiency,10)
(Maintainability,8.6)
(Portability,9.8)
(Security,10)
};
\legend{Product A, Product B, Product C, Product D, Product E}
\end{axis}
\end{tikzpicture}%


==> tex/ParResults.tex <==
\pgfplotsset{width=18cm,compat=1.14}
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.10,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={Weighted Score},
    symbolic x coords={1.1,1.2,1.3,1.4,1.5,1.6,1.7,1.8,2.1,2.2,2.3,2.4,2.5,2.6,3.1,3.2,3.3,3.4,3.5,3.6,4.1,4.2,4.3,4.4,5.1,5.2,5.3,5.4,5.5},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {
(1.1,2.8)
(1.2,2)
(1.3,2.8)
(1.4,0)
(1.5,2.8)
(1.6,2.8)
(1.7,0.396)
(1.8,1.876)
(2.1,3)
(2.2,0)
(2.3,3)
(2.4,0)
(2.5,3)
(2.6,4)
(3.1,0)
(3.2,2.8)
(3.3,2.8)
(3.4,0)
(3.5,1.254)
(3.6,0)
(4.1,5.6)
(4.2,0)
(4.3,0)
(4.4,0)
(5.1,3)
(5.2,2.5)
(5.3,1.25)
(5.4,0)
(5.5,3)
};
\addplot coordinates {
(1.1,2.8)
(1.2,2)
(1.3,2.8)
(1.4,0)
(1.5,2.8)
(1.6,2.8)
(1.7,0.396)
(1.8,1.876)
(2.1,3)
(2.2,0)
(2.3,3)
(2.4,0)
(2.5,3)
(2.6,4)
(3.1,0)
(3.2,2.8)
(3.3,2.8)
(3.4,0)
(3.5,1.254)
(3.6,0)
(4.1,5.6)
(4.2,0)
(4.3,0)
(4.4,0)
(5.1,3)
(5.2,2.5)
(5.3,1.25)
(5.4,0)
(5.5,3)
};
\addplot coordinates {
(1.1,2.8)
(1.2,2)
(1.3,2.8)
(1.4,0)
(1.5,2.8)
(1.6,2.8)
(1.7,0.396)
(1.8,1.876)
(2.1,3)
(2.2,0)
(2.3,3)
(2.4,0)
(2.5,3)
(2.6,4)
(3.1,0)
(3.2,2.8)
(3.3,2.8)
(3.4,0)
(3.5,1.254)
(3.6,0)
(4.1,5.6)
(4.2,0)
(4.3,0)
(4.4,0)
(5.1,3)
(5.2,2.5)
(5.3,1.25)
(5.4,0)
(5.5,3)
};
\addplot coordinates {
(1.1,2.8)
(1.2,2)
(1.3,2.8)
(1.4,0)
(1.5,2.8)
(1.6,2.8)
(1.7,0.396)
(1.8,1.876)
(2.1,3)
(2.2,0)
(2.3,3)
(2.4,0)
(2.5,3)
(2.6,4)
(3.1,0)
(3.2,2.8)
(3.3,2.8)
(3.4,0)
(3.5,1.254)
(3.6,0)
(4.1,5.6)
(4.2,0)
(4.3,0)
(4.4,0)
(5.1,3)
(5.2,2.5)
(5.3,1.25)
(5.4,0)
(5.5,3)
};
\addplot coordinates {
(1.1,2.8)
(1.2,2)
(1.3,2.8)
(1.4,0)
(1.5,2.8)
(1.6,2.8)
(1.7,0.396)
(1.8,1.876)
(2.1,3)
(2.2,0)
(2.3,3)
(2.4,0)
(2.5,3)
(2.6,4)
(3.1,0)
(3.2,2.8)
(3.3,2.8)
(3.4,0)
(3.5,1.254)
(3.6,0)
(4.1,5.6)
(4.2,0)
(4.3,0)
(4.4,0)
(5.1,3)
(5.2,2.5)
(5.3,1.25)
(5.4,0)
(5.5,3)
};
\legend{Product A, Product B, Product C, Product D, Product E}
\end{axis}
\end{tikzpicture}


==> tex/ProdResults.tex <==
\pgfplotsset{width=15cm,compat=1.14}
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.10,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={Weighted Score},
    symbolic x coords={Product A, Product B, Product C, Product D, Product E},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {
(Product A,15.472)
(Product B,12.304)
(Product C,8.5)
(Product D,16.496)
(Product E,15.304)
};
\addplot coordinates {
(Product A,13)
(Product B,9.25)
(Product C,8.25)
(Product D,12.5)
(Product E,10)
};
\addplot coordinates {
(Product A,6.854)
(Product B,3.946)
(Product C,5.6)
(Product D,20)
(Product E,8.6)
};
\addplot coordinates {
(Product A,5.6)
(Product B,16.8)
(Product C,6.552)
(Product D,18.6)
(Product E,9.8)
};
\addplot coordinates {
(Product A,9.75)
(Product B,11.5)
(Product C,4)
(Product D,3.75)
(Product E,10)
};
\legend{Reliability,Performance efficiency, Maintainability, Portability, Security}
\end{axis}
\end{tikzpicture}


==> tex/anonymized.tex <==
\usepackage{soul}
\sethlcolor{black}
%%\renewcommand{\hl}[1]{#1}
%\newcommand{\hl}[1]{#1}
\author{%
\IEEEauthorblockN{\hl{XxxxxXxxXxxxxx \quad XxxxxxXxxXxxxxx}}
\IEEEauthorblockA{\hl{\textit{XxxxxxxxxXxxxxxxxxxxxxxxxXxxxxxxxxXxxxxxx}}\\
\hl{\textit{XxxxXxxxxXxxxxxxxxxxxxxXxxxxx}}\\
\hl{XxxxxxxxxxXxxxxx}\\
\hl{Xxxxxxxxxxxxxxxxxx}}
}


==> tex/tikz_AOP2.tex <==
\pgfmathsetmacro{\myinnersep}{2}% inner sep in mm
%
\tikzset{%
	align=center,
	node distance=0.5cm and 0.1cm,
	ar/.style={->,>=latex},
%activity/.style={circle split,
activity/.style={circle,
%		every text node part/.style={font=\itshape},
%		every lower node part/.style={font=\footnotesize},
%line width=10mm,
%minimum width =5cm,
		text width=1.6cm,
		%%minimum height=0.5cm,
		%%text width=2.0cm,
		%minimum size=1cm,
		align=center,
		draw=black!80,
		fill=yellow!5,
		font=\scriptsize,
	},
	datastore/.style={trapezium,
		text width=1.9cm,
		%minimum height=0.5cm,
		%minimum height=1.0cm+4mm,
		%minimum size=2cm,
		%minimum width=0.4cm,
		%text height=0.5cm,
		%text height=1.04cm,
		%%minimum width=2.0cm,
		%%text width=1.8cm,
		align=center,
		draw=blue!60,
		fill=green!5,
		font=\scriptsize,
		inner sep=2,
		outer sep=0,
		shape=trapezium,
		trapezium left angle=70,
		trapezium right angle=110,
	},
}
%
\begin{tikzpicture}[%
]
\node[datastore,
%		text width=1.8cm,
		%%text width=2.2cm,
		%%minimum width=2.0cm,
%		minimum height=0.5cm,
%		text height=0.5cm,
%		minimum size=2cm,
%		minimum width=0.4cm,
%		minimum height=1.0cm+4mm,
]  (b1) {\BOX{\BYPRODUCT{1};\BYPRODUCT{3}}\\Possible Architectures};

\node[activity,above=of b1] (a1) {%
%	$1.0$\\[-2.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
	\\[-2.5\baselineskip]$1.0$\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
%	\nodepart{lower}
	\BOX{\ActivityI;\ActivityIII}\\Architecture Generation
%
%\draw (0,+1.4) node[fill=white]{a Top Piece b};
%\draw (0,-0.5) node[fill=white]{c\quad Bottom Piece\quad d};
};

%  \node [circle split,
%         draw,
%         minimum width=4cm,
%         append after command={%
%          let \p1=($(\tikzlastnode.east)-(\tikzlastnode.west)$) in  
%              node[draw,
%                   shape=semicircle,
%                   rotate=180,
%                   anchor=south,
%                   double,
%                   minimum width=\x1] at (\tikzlastnode.center)     {}}]
%  {top
%    \nodepart{lower}
%    below
%  };
%
%\node[ultra thick, red, draw]
% at (+1,+1)
%  (x1)[text=blue] {I am};


\node[datastore,right=of b1] (b2) {\BOX{\BYPRODUCT{2};\BYPRODUCT{4}}\\Suitability and Quality Gaps};

\node[activity,above=of b2] (a2) {%
	\\[-2.5\baselineskip]$2.0$\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
%	\nodepart{lower}
	\BOX{\ActivityII;\ActivityIV}\\Architecture Evaluation
};

\node[datastore,above=of a2,minimum width=5.0cm,text width=5.0cm]
	(ir) {\IR\\Requirements\\(Functional, Quality, Constraints)};

\node[datastore,right=of b2] (oa) {\OA\\Optimal Architecture};

\node[activity,above=of oa] (a5) {%
	\\[-2.5\baselineskip]$3.0$\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
%	\nodepart{lower}
	\BOX{\ActivityV}\\Architecture Selection
};

\draw[ar,bend left,xshift=-0.5cm]
  (a1) edge (b1);
\draw[ar,bend left,xshift=0.5cm] 
  (b1) edge (a1);
\draw[ar] 
  (b1) edge (a2);
\draw[ar] 
  (a2) -- (b2);
\draw[ar] 
  (b2) -- (a1);
\draw[ar] 
  (b2) -- (a5) node[pos=0.5]{/};
\draw[ar] 
  (a5) -- (oa);
\draw[ar]
  (ir) -- (a1);
\draw[ar]
  (ir) -- (a2);
\draw[ar] 
  (b1) -- (a5) node[pos=0.8]{/};
%\draw[ar,xshift=1.5cm,yshift=1.5cm] 
%  (b1) .. controls (right:1.5cm).. (a5);
%  (b1) .. controls +(up:1.5cm) and (right:1.5cm).. (a5);
%\draw[ar,bend right,yshift=0.5cm] 
%  (b1.east) edge (a5);
%\draw[ar,bend right] 
%  (b1.east) .. controls +(down:1cm) and +(right:1cm) .. (a5);
%  (b1) .. controls +(up:1cm) and +(left:1cm) .. (a5);
\end{tikzpicture}


==> tikz/fig_AOE.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \centering
  \input{tikz_AOE}
  %\caption{The abstract structure of an AOE (flowchart)}
  \caption{Activities and byproducts in the \AOP.}
  \label{fig:AOE}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tikz/tikz_AOE.tex <==
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers
%\usetikzlibrary{positioning}
%\usetikzlibrary {shapes.geometric}
%\pgfdeclareshape{patastore}{
%  \inheritsavedanchors[from=rectangle]
%  \inheritanchorborder[from=rectangle]
%  \inheritanchor[from=rectangle]{center}
%  \inheritanchor[from=rectangle]{base}
%  \inheritanchor[from=rectangle]{north}
%  \inheritanchor[from=rectangle]{north east}
%  \inheritanchor[from=rectangle]{east}
%  \inheritanchor[from=rectangle]{south east}
%  \inheritanchor[from=rectangle]{south}
%  \inheritanchor[from=rectangle]{south west}
%  \inheritanchor[from=rectangle]{west}
%  \inheritanchor[from=rectangle]{north west}
%}
%
\begin{tikzpicture}[
	node
	distance=0.5cm and 0.8cm,
	ar/.style={->,>=latex},
	mycircle/.style={circle,
		font=\scriptsize,
		draw=magenta!60,
		fill=magenta!5,
		very thick,
		minimum size=7mm,
		text width=1.2cm,
		minimum height=1cm,
		align=center,
		},
	activity/.style={circle,
	font=\scriptsize,
	draw=black!80,
	%fill=yellow!5,
	rounded corners=3mm,
%	text width=2.5cm,
%	text width=1.5cm,
	text width=2.0cm,
	minimum height=0.5cm,
%	minimum size=1cm,
	align=center},
	datastore/.style={
		text width=1.9cm,
		draw=black!60,
		very thick,
		shape=datastore,
		font=\scriptsize,
		inner sep=2,
		outer sep=0,
		align=center,
	},
	datastores/.style={
		shape=trapezium,
		trapezium right angle=110,
		trapezium left angle=70,
		font=\scriptsize,
		%draw=blue!60,
		draw=black!60,
		%fill=blue!5,
		%fill=black!5,
%		text width=2.3cm,
		text width=2.2cm,
		minimum width=2.0cm,
%		minimum height=1cm,
%%		text height=0.5cm,
%		minimum size=2cm,
		align=center,
		},
%	datastore/.style={draw,very thick,shape=datastorestore,inner sep=.3cm},
	mylabel/.style={
		rectangle,
		font=\scriptsize,
		draw=yellow!0,
		fill=yellow!0,
%		text width=2.5cm,
%		minimum height=1cm,
		align=center,
		},
]

%\node[mycircle] (ss) {START};
\node[datastore,label=below:{\scriptsize\BYPRODUCT{1}}] (b1) {Initial Architecture% (1)
};
%%%
%%% 2.1
%%%
\node[activity,above=of b1,fill=black!5] (a1) {%
	\\[-2.5\baselineskip]\DFD{2.1}\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
\ActivityI\\\sc Initial Architecture Creation% (0$\,\to\,$1)
};
\node[datastore,right=of b1,minimum width=2.3cm,text width=2.    3cm,label=below:{\scriptsize\BYPRODUCT{2}}] (b2) {Initial Suitability and Quality Gaps% (1)
};
\node[datastore,right=of b2,label=below:{\scriptsize\BYPRODUCT{3}}] (b3) {Alternative Architectures% (N)
};
%%%
%%% 1.1
%%%
\node[activity,above=of b3,fill=black!29] (a2) {
	\\[-2.5\baselineskip]\DFD{1.1}\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
\ActivityII\\\sc Initial Architecture Evaluation% (1)
};
%%%
%%% 2.2
%%%
\node[activity,above=of b2,fill=black!7] (a3) {
	\\[-2.5\baselineskip]\DFD{2.2}\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
\ActivityIII\\\sc Alternative Architectures Creation% (1$\,\to\,$N)
};
%\node[datastore,above=of a3] (ir) {\NODESTYLE{IR} Requirements};
\node[datastore,above=of a2,minimum width=5.0cm,text width=5.0cm,label=above:{\scriptsize\IR}] (ir) {Requirements\\(Functional, Quality, Constraints)};
\node[datastore,right=of b3,label=below:{\scriptsize\BYPRODUCT{4}}] (b4) {Suitability and Quality Gaps% (N)
};
%%%
%%% 1.2
%%%
\node[activity,above=of b4,fill=black!29] (a4) {
	\\[-2.5\baselineskip]\DFD{1.2}\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
\ActivityIV\\\sc Alternative Architecture Evaluation% (N)
};
\node[datastore,right=of b4,label=below:{\scriptsize\OA}] (oa) {Optimal Architecture% (1)
};
%%%
%%% 3.0
%%%
\node[activity,above=of oa,fill=black!14] (a5) {
	\\[-2.5\baselineskip]\DFD{3.0}\\[-0.5\baselineskip]{\rule{\linewidth}{.4pt}}\\
\ActivityV\\\sc Optimal Architecture Selection% (N$\,\to\,$1)
};
%%%
\begin{pgfonlayer}{bg}    % select the background layer
\draw[black,thick,dotted,fill=black!5] ($(a1.north west)+(-0.5,0.6)$) rectangle ($(a3.south east)+(0.5,-0.3)$); % node (YY) {YYYYY};
\node (proc) at ([shift={(6.0:1.3)}]$(a1.north west)+(-0.5,0.3)$) [align=left] {\scriptsize Architecture~Generation};
\draw[black,thick,dotted,fill=black!5] ($(a2.north west)+(-0.5,0.6)$) rectangle ($(a4.south east)+(0.5,-0.3)$); % node (YY) {YYYYY};
\node (proc) at ([shift={(6.0:1.3)}]$(a2.north west)+(-0.5,0.3)$) [align=left] {\scriptsize Architecture~Evaluation};
\draw[black,thick,dotted,fill=black!5] ($(a5.north west)+(-0.5,0.6)$) rectangle ($(a5.south east)+(0.5,-0.3)$); % node (YY) {YYYYY};
\node (proc) at ([shift={(6.0:1.3)}]$(a5.north west)+(-0.5,0.3)$) [align=left] {\scriptsize Architecture~Selection};
\end{pgfonlayer}
%%%
%\node[mycircle,below=of oa] (ee) {END};
%
%\node[mylabel,below=of a4] (l1) {Legend:};
%\node[activity,right=of l1] (l2) {Activity};
%\node[datastore,right=of l2] (l3) {Data};
%
%\draw[ar] 
%  (ss) -- (ir);
%\draw[ar] 
%  (ir) -- (a1);
\draw[ar] 
  (a1) -- (b1);
\draw[ar] 
  (b1) -- (a2);
\draw[ar] 
  (a2) -- (b2);
\draw[ar] 
  (b2) -- (a3);
\draw[ar] 
  (a3) -- (b3);
\draw[ar] 
  (b3) -- (a4);
\draw[ar] 
  (a4) -- (b4);
\draw[ar] 
  (b4) -- (a5);
\draw[ar] 
  (a5) -- (oa);
%\draw[ar] 
%  (oa) -- (ee);
\draw[ar] 
  (ir) -- (a2);
%\draw[ar] 
%  (ir) -- (a4);
%\draw[rectangle] (ir) to (a2);
%\draw[ar] (ir) -- +(0,2) |- (a2);
\draw[ar] (ir) -- +(-3,0) to (a1);
\draw[ar] (ir) -- +(+3,0) to (a4);
\draw[ar] 
  (b3) -- (a5);
%
%
%
%\draw[ar] 
%  (ie) -- node[above] {d} (db);
%\draw[ar] 
%  (db) -- node[above] {e} (ec);
%\draw[ar] 
%  (ec) -- node[above] {f} (ee);
%\draw[ar] 
%  (ee.70) to[out=120,in=0] node[above] {c} (ai.east);
%\draw[ar] 
%  (ai.west) to[out=180,in=90] node[left] {b,c} (ie.130);
%\draw[ar] 
%  (ee.120) to[out=170,in=90,looseness=1.3] %node[pos=0.93,left=3pt] {a} (db.north);
%\draw[ar] 
%  (ec.120) to[out=100,in=-20] node[pos=0.1,left=3pt] {b} %(ai.east);
%\draw[ar] 
%  (ie.320) to[out=-40,in=200] node[pos=0.87,right=12pt] {i} %(ee.south);
%\draw[ar] 
%  (ie.320) to[out=-40,in=230] node[pos=0.87,right=6pt] {h} %(ec.south);
\end{tikzpicture}

